HLS-Eval: A Benchmark and Framework for Evaluating LLMs on High-Level Synthesis Design Tasks

The rapid scaling of large language model (LLM) training and inference has driven their adoption in semiconductor design across academia and industry. While most prior work evaluates LLMs on hardware description language (HDL) tasks, particularly Verilog, designers are increasingly using high-level synthesis (HLS) to build domain-specific accelerators and complex hardware systems. However, benchmarks and tooling to comprehensively evaluate LLMs for HLS design tasks remain scarce. To address this, we introduce HLS-Eval, the first complete benchmark and evaluation framework for LLM-driven HLS design. HLS-Eval targets two core tasks: (1) generating HLS code from natural language descriptions, and (2) performing HLS-specific code edits to optimize performance and hardware efficiency. The benchmark includes 94 unique designs drawn from standard HLS benchmarks and novel sources. Each case is prepared via a semi-automated flow that produces a natural language description and a paired testbench for C-simulation and synthesis validation, ensuring each task is "LLM-ready." Beyond the benchmark, HLS-Eval offers a modular Python framework for automated, parallel evaluation of both local and hosted LLMs. It includes a parallel evaluation engine, direct HLS tool integration, and abstractions for to support different LLM interaction paradigms, enabling rapid prototyping of new benchmarks, tasks, and LLM methods. We demonstrate HLS-Eval through baseline evaluations of open-source LLMs on Vitis HLS, measuring outputs across four key metrics - parseability, compilability, runnability, and synthesizability - reflecting the iterative HLS design cycle. We also report pass@k metrics, establishing clear baselines and reusable infrastructure for the broader LLM-for-hardware community. All benchmarks, framework code, and results are open-sourced at https://github.com/stefanpie/hls-eval.

==> prompts/meta_code_file.tex <==
\begin{prompt}
File Name: `{file_name}`
```{md_code_block_type}
{file_contents}
```
\end{prompt}

==> prompts/meta_extract.tex <==
\begin{prompt}
You are a high-level synthesis expert.
Help me extract the code for a specific sub-component in this high-level synthesis hardware design."
       
Given the existing kernel code, header, and optional description, extract the code for a specific sub-component in the design.
A sub-component is a separate C++ function in the code that is not the top-level function.
       
The top level HLS kernel function is: `{top_name}`

The sub-component to extract is: `{subcomponent_name}`

Only output the code in a single C++ code block that contains the code for the sub-component and all additional code needed to compile and run the sub-component (including other sub-components called by target sub-component).
Assume you can use the same header file and any other code in the directory to compile and run the sub-component.
Do not include the `cpp` identifier in the markdown code block, just the code block ticks.
       
The output should be formatted exactly follows with no deviation:
```
C++ code for the sub-component...
```
       
Optional pre-existing simple kernel_description.md file:
       
{existing_description}
       
Input Kernel Code:

{kernel_code}
       
Code for the Sub-Component in requested C++ code block format (do not provide anything other than the code for the sub-component in the requested format):
\end{prompt}
